Artificial Intelligence for Satellite Communication and Non-Terrestrial Networks: A Survey

This paper surveys the application and development of Artificial Intelligence (AI) in Satellite Communication (SatCom) and Non-Terrestrial Networks (NTN). We first present a comprehensive list of use cases, the relative challenges and the main AI tools capable of addressing those challenges. For each use case, we present the main motivation, a system description, the available non-AI solutions and the potential benefits and available works using AI. We also discuss the pros and cons of an on-board and on-ground AI-based architecture, and we revise the current commercial and research activities relevant to this topic. Next, we describe the state-of-the-art hardware solutions for developing ML in real satellite systems. Finally, we discuss the long-term developments of AI in the SatCom and NTN sectors and potential research directions. This paper provides a comprehensive and up-to-date overview of the opportunities and challenges offered by AI to improve the performance and efficiency of NTNs.

==> acronyms.tex <==
\begin{acronym} 
\acro{3G}{Third Generation}
\acro{4G}{Fourth Generation}
\acro{5G}{Fifth Generation}
\acro{6G}{sixth generation}
\acro{3GPP}{3rd Generation Partnership Project}
\acro{ACO}{Ant Colony Optimization}
\acro{ACM}{Adaptive Coding and Modulation}
\acro{AI}{Artificial Intelligence}
\acro{ANN}{Artificial Neural Network}
\acro{AoI}{Age of Information}
\acro{BB}{Base Band}
\acro{BBU}{Base Band Unit}
\acro{BC}{Blockchain}
\acro{BER}{Bit Error Rate}
\acro{BH}{Beam Hopping}
\acro{BS}{Base Station}
\acro{BW}{bandwidth}
\acro{C-RAN}{Cloud Radio Access Networks}
\acro{CAPEX}{Capital Expenditure}
\acro{CDMA}{Code Division Multiple Access}
\acro{CN}{Core Network}
\acro{CNN}{Convolutional Neural Network}
\acro{CoMP}{Coordinated Multipoint}
\acro{CR}{Cognitive Radio}
\acro{CSI}{Channel State Information}
\acro{D2D}{Device-to-Device}
\acro{DAC}{Digital-to-Analog Converter}
\acro{DAS}{Distributed Antenna Systems}
\acro{DBA}{Dynamic Bandwidth Allocation}
\acro{DC}{Duty Cycle}
\acro{DL}{Deep Learning}
\acro{DNN}{Deep Neural Network}
\acro{DBF}{Digital Beam Forming}
\acro{DPD}{Digital Predistortion}
\acro{DRAA}{Direct Radiating Active Antennas}
\acro{DQL}{Deep Q-learning}
\acro{DRL}{Deep Reinforcement Learning}
\acro{DSA}{Dynamic Spectrum Access}
\acro{DSS}{Dynamic Spectrum Sharing}
\acro{DT}{Decision Tree}
\acro{DU}{Deep Unfolding}
\acro{EO}{Earth Observation}
\acro{ESA}{European Space Agency}
\acro{EIRP}{Effective Isotropic Radiated Power}
\acro{FBMC}{Filterbank Multicarrier}
\acro{FDMA}{Frequency Division Multiple Access}
\acro{FEC}{Forward Error Correction}
\acro{FL}{federated learning}
\acro{FFR}{Fractional Frequency Reuse}
\acro{FSO}{Free Space Optics}
\acro{GA}{Genetic Algorithms}
\acro{GAN}{Generative Adversarial Network}
\acro{GCN}{Graph Convolutional Network}
\acro{GEO}{Geo-Stationary Orbit}
\acro{GS}{Ground Segment}
\acro{GSD}{Ground Segment Dimensioning}
\acro{GSO}{Geosynchronous Orbit}
\acro{GW}{Gateway}
\acro{HAP}{High Altitude Platform}
\acro{HL}{Higher Layer}
\acro{HARQ}{Hybrid-Automatic Repeat Request}
\acro{HCA}{Hierarchical Cluster Analysis}
\acro{HO}{Handover}
\acro{HTS}{High Throughput Satellites}
\acro{KNN}{k-nearest neighbors}
\acro{KPI}{Key Performance Indicator}
\acro{IoT}{Internet of Things}
\acro{JCS}{Joint Communication and Sensing}
\acro{ISAC}{Integrated Sensing and Communication}
\acro{LA}{Link Adaptation}
\acro{LAN}{Local Area Network}
\acro{LAP}{Low Altitude Platform}
\acro{LDPC}{Low-Density Parity-Check} 
\acro{LEO}{Low Earth Orbit}
\acro{LL}{Lower Layer}
\acro{LoS}{Line of Sight}
\acro{LP}{Linear Precoding}
\acro{LTE}{Long Term Evolution}
\acro{LTE-A}{Long Term Evolution Advanced}
\acro{LSTM}{long short-term memory}
\acro{MAC}{Medium Access Control}
\acro{MaD-DPD}{Memory Polynomial aided Deep Neural Network Digital Predistortion}
\acro{MAP}{Medium Altitude Platform}
\acro{MEC}{Mobile Edge Computing}
\acro{MDP}{Markov Decision Process}
\acro{MODCOD}{Modulation and Coding}
\acro{MMSE}{Minimum Mean-Square Error}
\acro{MPM}{Memory Polynomial}
\acro{MIMO}{Multiple-Input Multiple-Output}
\acro{ML}{Machine Learning}
\acro{MLP}{Multilayer Perceptron}
\acro{M2M}{Machine-to-machine}
\acro{mmWave}{millimeter Wave}
\acro{NEC}{Neural Episodic Control} 
\acro{NFP}{Network Flying Platform}
\acro{NFV}{Network Function Virtualization}
\acro{NGSO}{Non Geo-Stationary}
\acro{NN}{Neural Network}
\acro{NOMA}{Non-orthogonal Multiple Access}
\acro{NR}{New Radio}
\acro{NTN}{Non-Terrestrial Network}
\acro{OFDM}{Orthogonal Frequency-division Multiplexing}
\acro{OFDMA}{Orthogonal Frequency-Division Multiple Access}
\acro{OGS}{Optical Ground Station}
\acro{OMA}{Orthogonal Multiple Access}
\acro{OPEX}{Operational Expenditure}
\acro{ORRF}{Online Random Regression Forest} 
\acro{OBO}{Output Back-Off}
\acro{PA}{Power Amplifier}
\acro{PAM}{Pulse Amplitude Modulation}
\acro{PGD}{Projection Gradient Descent}
\acro{PSO}{Particle Swarm Optimization}
\acro{QoE}{Quality of Experience}
\acro{QoS}{Quality of Service}
\acro{RAN}{Radio Access Network}
\acro{RDN}{residual dense network} 
\acro{RF}{Radio Frequency}
\acro{RL}{Reinforcement Learning}
\acro{RRM}{Radio Resource Management}
\acro{RS}{Remote Sensing}
\acro{RTT}{Round Trip time}
\acro{RZF}{Regularized Zero Forcing}
\acro{SAGIN}{Space-Air-Ground Integrated Network}
\acro{SATCOM}{Satellite Communication}
\acro{SCBS}{Small Cell Base Station}
\acro{SDMA}{Spaced Division Multiple Access}
\acro{SDN}{Software Defined Network}
\acro{SE}{Spectral Efficiency}
\acro{SIC}{Successive Interference Cancellation}
\acro{SIP}{Satellite Image Processing} 
\acro{SLL}{Side Lobe Level}
\acro{SNR}{Signal-to-Noise Ratio}
\acro{SON}{Self-organising Network}
\acro{ST}{Satellite Terminal}
\acro{SSPA}{Solid-State Power Amplifier}
\acro{SV}{Satellite Video} 
\acro{SVC}{Support Vector Classifier}
\acro{PAE}{Power-Added Efficiency}
\acro{PEP}{Peak Envelope Power}
\acro{PAPR}{Peak-to-Average Power Ratio}
\acro{SVM}{Support Vector Machine}
\acro{TDM}{Time Division Multiplexing}
\acro{TDMA}{Time Division Multiple Access}
\acro{TWTA}{Traveling-Wave Tube Amplifiers}
\acro{NTN}{Non Terrestrial Network}
\acro{TN}{Transport Network}
\acro{UAV}{Unmanned Aerial Vehicle}
\acro{UHTS}{Ultra High Throughput Satellites}
\acro{UE}{User Equipment}
\acro{PoP}{Point of Presence}
\acro{OAI}{OpenAirInterface}
\acro{TEG}{time-expanded graph}

%%%%%% Antenna Design%%%%%
\newacro{FDTD}{Finite-difference time-domain method}
\newacro{FEM}{Finite element method}
\newacro{GO}{Geometric optics}
\newacro{PO}{Physical optics}
\newacro{MoM}{Method of Moments}
%%%%%%%
\newacro{SCS}{satellite communication system}
\newacro{NCC}{network control centre}
\newacro{SKC}{secret-key cryptosystem}
\newacro{PKC}{public-key cryptosystem}
\newacro{GNSS}{global navigation satellite system}
\newacro{RNN}{recurrent neural network}
\newacro{LEO}{low-earth orbit}
\newacro{PLS}{physical-layer security}
%\newacro{MIMO}{multiple-input multiple-output}
\newacro{QKD}{quantum key distribution}

\newacro{DRT}{dehop-rehop transponder}
\newacro{FH-FDMA}{frequency hopping-frequency division multiple access}
\newacro{LO}{local oscillator}
\newacro{TLL}{timing locked loop}
\newacro{TCL}{timing control loop}
\newacro{RBF}{radial basis function neural network}
\newacro{PNN}{probabilistic neural network}
\newacro{ABF}{adaptive beam forming}

\newacro{NCO}{numerically-controlled oscillator}
\newacro{VCO}{voltage-controlled oscillator}
%%%
\newacro{NAS}{Neural Architecture Search}
\newacro{MILP}{Mixed-Integer Linear Programming}
%%%%%%%%%%%%
\end{acronym}






==> coverLetter.tex <==
Dear Editors:
We would like to submit the enclosed manuscript entitled “Artificial Intelligence for Satellite Communication and Non-Terrestrial Networks: A Survey”, which we wish to be considered for publication in IEEE Communications Surveys & Tutorials. No conflict of interest exits in the submission of this manuscript, and manuscript is approved by all authors for publication. I would like to declare on behalf of my co-authors that the work described was original research that has not been published previously, and not under consideration for publication elsewhere, in whole or in part. All the authors listed have approved the manuscript that is enclosed.
The submitted survey has the following abstract:
This paper surveys the application and development of Artificial Intelligence (AI) in Satellite Communication (SatCom) and Non-Terrestrial Networks (NTN). We first present a comprehensive list of use cases, the relative challenges and the main AI tools capable of addressing those challenges. For each use case, we present the main motivation, a description of the system, the available non-AI solutions and the potential benefits and available works using AI. We also present a discussion on the pros and cons of an on-board and on-ground AI-based architecture and we revise the current commercial and research activities relevant to this topic. Next, we describe the state-of-the-art hardware solutions for developing ML in real satellite systems. Finally, we discuss the long-term developments of AI in the SatCom and NTN sector and potential research directions. This paper provides a comprehensive and up-to-date overview of the opportunities and challenges offered by AI to improve the performance and efficiency of NTNs.


We deeply appreciate your consideration of our manuscript, and we look forward to receiving comments from the reviewers. If you have any queries, please don’t hesitate to contact me at the address below.
Thank you and best regards.
Yours sincerely,
Gianluca Fontanesi

Corresponding author:
Name: Gianluca Fontanesi 
E-mail: gianluca.fontanesi@nokia.com

